Towards Practical Finite Sample Bounds for Motion Planning in TAMP

When using sampling-based motion planners, such as PRMs, in configuration spaces, it is difficult to determine how many samples are required for the PRM to find a solution consistently. This is relevant in Task and Motion Planning (TAMP), where many motion planning problems must be solved in sequence. We attempt to solve this problem by proving an upper bound on the number of samples that are sufficient, with high probability, to find a solution by drawing on prior work in deterministic sampling and sample complexity theory. We also introduce a numerical algorithm to compute a tighter number of samples based on the proof of the sample complexity theorem we apply to derive our bound. Our experiments show that our numerical bounding algorithm is tight within two orders of magnitude on planar planning problems and becomes looser as the problem's dimensionality increases. When deployed as a heuristic to schedule samples in a TAMP planner, we also observe planning time improvements in planar problems. While our experiments show much work remains to tighten our bounds, the ideas presented in this paper are a step towards a practical sample bound.

==> sections/legacy/experiments_optimality.tex <==
We seek to experimentally verify the tightness of our sampling bound of convergence to path feasibility and optimality as computed by Algorithm \ref{alg:numerical_complexity}. 
Our results are found in Table \ref{tab:uni-clear-opt}.

\subsection{Clearance Experiments}
Our clearance experiments are conducted in a `narrow hallway' problem that can be generalized to arbitrarily high dimensions.
The configuration space can be characterized by 
$$
\underbrace{\paren{[-1.5, -0.5] \times [-0.5, 0.5]^{d-1}}}_{\text{"left" end}} \cup 
\underbrace{\paren{[-0.5, 0.5] \times [-\delta, \delta]^{d-1}}}_{\text{hallway}} \cup 
\underbrace{\paren{[0.5, 1.5] \times [-0.5, 0.5]^{d-1}}}_{\text{"right" end}}.
$$

We construct many instances of this hallway problem for varying $\delta < 0.5$ and for $d = \{2, 3, 6, 7, 14, 20\}$. To estimate the probability of success, we run a Monte-Carlo estimate and then check if the PRM is $(\delta, \infty)$-complete (Appendix \ref{sec:set_cover}) in the narrow passage region.
We note that we are not checking the full $(\epsilon,\delta$-completeness condition -- we need to verify the existence of PRM solutions for paths in the hallway "ends" if we did -- but it is computationally infeasible to do so.
The estimated probability will form an upper bound on the probability of $(\delta, \infty)$-completeness, since a positive MC-iteration may confirm that paths exist in the hallway, but may not for the ends.
We observe that the bound is shockingly tight in all dimensions (\sas{I'm inferring from from low-dimensional trial runs, and high-dim exps are usually tighter, but those experiments are still running at the moment.}).



\subsection{Optimality Experiments}
Our optimality experiments are conducted in a simple "box" environment $[-\delta, 1 + \delta] \times [-\delta, \delta]^{d-1} \subset \R^d$ where $\delta$ is a fixed clearance. 
The optimal $\delta$-clear path is a single-component subset of $[0, 1] \times \{0\}^{d-1}$.
Our experiments attempt to estimate the probability of failure as a function of optimality tolerance $\epsilon$ by running a large number of Monte-Carlo trials.

To efficiently run a single trial of $m$ i.i.d samples, we make two observations. First, the optimality factor has a strictly monotonic relationship with the required connection radius in the hypothesis of Theorem \ref{thm:rough_sample_bound}: 
$\epsilon \mapsto 2\delta \cdot (1 + \epsilon) / \sqrt{1+\epsilon^2}=r$ when $\epsilon \in [0, 1]$.
Second, if $r < r'$ are two connection radii, then given the same set of samples, a PRM with connection radius $r$ is always a subgraph of a PRM with connection radius $r'$.

Let $\epsilon < \epsilon'$ be two tolerances, and $r < r'$ their associated connection radii.
Let $\ell_r$ and $\ell_{r'}$ be the lengths of some motion planning solution with the same start and goal to $r$-PRM and $r'$-PRM respectively.
Suppose the optimal $\delta$-clear path has length $\ell$.
If both PRMs, are $(\epsilon^{(\prime)}, \delta)$-complete with respect to their radii, then
$$
\ell_r' \leq \ell_r < (1 + \epsilon) \cdot \ell  < (1 + \epsilon') \cdot \ell
$$
Thus, for a single MC-iteration, we can check for completeness \textit{for all $\epsilon \in [0, 1]$} \footnote{The memory limits of the computer running in the algorithm places an upper bound on the connection radius of the graph, and thus an upper bound on the $\epsilon$ we are able to check.} by performing throwing away edges (in length) in a binary search fashion, computing the associated optimality tolerance for the `effective' connection radius of the graph, and then checking for completeness for that tolerance.
We check for $(\epsilon, \delta)$-completeness by solving for a (non-miminal) set-cover over the set of possible starts and goals of the $\delta$-optimal path (Appendix \ref{sec:set_cover}).

We observe that our bound is loose by slightly more than a constant factor, which makes sense since the bound makes a pessimistic estimate of the placement of the points in the $\rho$-transversal constructed in Theorem \ref{thm:rough_sample_bound}.




\begin{table}[h]
\parbox{0.3\linewidth}{
    \begin{tabular}{|l|l|}
        \hline
         & Increasing $1 / \epsilon \rightarrow$  \\
        \hline
        \rotatebox[origin=c]{90}{$\leftarrow$ Increasing dimension $d$} & \makecell{Increase linearly $\rightarrow$,\\ Increase exp. $\downarrow$ }\\
        \hline
    \end{tabular}
}
\hfill
\parbox{0.3\linewidth}{
    \begin{tabular}{|l|l|}
        \hline
         & Increasing $1 / \delta \rightarrow$  \\
        \hline
        \rotatebox[origin=c]{90}{$\leftarrow$ Increasing dimension $d$} & \makecell{Increase linearly $\rightarrow$,\\ Increase exp. $\downarrow$ }\\
        \hline
    \end{tabular}
}
\hfill
\parbox{0.3\linewidth}{
    \begin{tabular}{|l|l|}
        \hline
         & Increasing $1 / \gamma \rightarrow$  \\
        \hline
        \rotatebox[origin=c]{90}{$\leftarrow$ Increasing dimension $d$} & \makecell{Increase log. $\rightarrow$,\\ No change $\downarrow$ }\\
        \hline
    \end{tabular}
}
\caption{Predicted (adjusted by a constant factors) and computed complexities for environments of varying clearance or optimality (predicted by theory).}\label{tab:uni-clear-opt}
\end{table}







==> sections/legacy/extra_bits.tex <==
\subsection{Outline of Sample Complexity Proof, and Deriving a Tighter Numerical Algorithm}
% Preamble (changeup from nb): we take advantage of results from computational learning theory to derive our bounds often used in scenarios of probably-approximately correct machine learning.

We leverage sample-complexity bounds from probabably-approximately correct (PAC) learning to derive our sample bounds.
Our results analogizes motion planning to machine learning by re-interpreting our random samples as our `data'.
As done in in PAC-learning, we want to analyze the probability that a set of random samples from a uniform distribution fall in a desirable configuration for the PRM admit the "$\delta$-wide path guarantee" with high probability. \sas{better way to write this last sentence? not sure yet.}

A key insight by Janson et al. \cite{janson_deterministic_2018} and Tsao et al. \cite{tsao_sample_2019} is that deterministic sample sequence that forms a  `ball-covering' (or low-dispersion set) with a suitable connection radius can yield a PRM that will contain a solution within a tube of a path with clearance $\delta$ (a $\delta$-tube, in fact).
Our bounds analyze that probability that a random sample set form the same type of covering.

% then take advtange of the fact that Blumer's proof is a proof by the probabilistic method.
Luckily, random coverings have been well-studied by computational learning theorists and discrete geometers, who were interested in constructing coverings with sets with geometry more general than spheres.
Usually, these covering bounds are stated in terms of the smallest covering available \cite{komlos_almost_1992}, but Blumer et al. attempt to estimate the probability that the samples form a covering \cite{blumer_learnability_1989}.
We opt to use the results from latter to understand the asymptotic scaling of the data (read: samples) required with respect to the probability of failing to find a covering $\gamma$.

While the bound stated in \cite{blumer_learnability_1989,komlos_almost_1992} are tight up to constant factors\footnote{These results are tight up to a special constant that Blumer et al. and Komlos et al. use as an abstration over coverings with specific geometries (half-planes, balls, triangles etc.), called the Vapnik-Chervonenkis dimension \cite{matousek_lectures_2002,mustafa_sampling_2022}. It may very well be true that one may prove tighter bounds if we can exploit the geometry of these sets. See Appendix for more details.}, 
using the exact mathematical equations presented in the statement of the theorems results in loose over-approximations of true number of samples.
We exploit the fact that common technique these covering constructions \cite{vapnik_uniform_1971,blumer_learnability_1989,komlos_almost_1992} are proved using the probabilistic method to derive a numerical algorithm that, given a planning problem, narrow passage width, and failure probability, computes a tighter (and theoretical sound) upper bound on the number of samples that is more useful in practice.


% The issue with abstract sequences -> refinement paradigms, and standard approaches to address them
There is a fundamental issue that must always be addressed in bilevel planning: not all abstract mode sequences can be refined into feasible motions \cite{hauser_integrating_2009}.
Sampling-based motion planners, such as Probabilistic Roadmaps (PRMs) \cite{kavraki_probabilistic_1996}, are widely used as the motion planning subroutines, but are known to never terminate when the input motion planning problem is infeasible.
In practice, many choose a maximum number of samples to be used by the sampling-based motion planner, and upon failing to find a solution between two mode transitions, the high level mode-sequencer can postpone the candidate mode sequence to be re-attempted later  \cite{hauser_integrating_2009,garrett_pddlstream_2020}.
Our goal to address this problem will proceed on a different (and perhaps, complementary) tack: we aim to estimate the probability that a feasible path does not exist as a function of the number of samples taken by the (PRM).



Constructing PRMs from deterministic sampling processes present  stronger guarantees available for finding a path, without assumptions of existence, and only path width (should they exist) , and faster convergence rates to optimality \cite{janson_deterministic_2018,tsao_sample_2019} .
Our bounds prove the probability of the events in the same manner as the deterministic sampling sequences, but are looser because sampling sequences have asymptotically weaker decay rates in the radius largest empty ball (sample `dispersion'; with high probability) than deterministic sequences \cite{niederreiter_random_1992}.

If we have stronger results for deterministic sampling procedures, why should we even consider bounds for random sampling procedures?
A shortcoming of the best performing (fastest dispersion decay rate) deterministic sequences is that the number and placement are all decided beforehand, given as input the collision-free configuration space and the largest desired empty ball (sample dispersion) \cite{niederreiter_random_1992,matousek_lectures_2002,janson_deterministic_2018}. 
Should the decision-maker want to construct a sequence for a smaller empty ball or the configuration space significantly change, the first sequence becomes moot and the motion planning algorithm must construct another sequence from scratch.
Random samples easier to implement and naturally incremental, so they are amenable to construct anytime motion planning algorithms. \sas{we'd have to justify why anytime is a good thing. and I have strong probabilistic reasons for why; but perhaps there is a simpler one? Would love to discuss.}

Our analysis bounds the number of samples sufficient for the PRM to 'approximate' paths of given width  $\delta$ (the clearance refers to the radius of a ball that can be `slid' along a feasible path that does not touch the obstacle set) and probability of the guarantee's failure $\gamma$.
We show that the number of samples varies exponentially in $1/\delta$, and logarithmically in $1/\gamma$.
Most importantly, should a motion planner decide to sample up to our probability bound and not find a path, then we can be certain that a path with width $\delta$ does not exist with at least probability $1 - \gamma$. 
The probability $1 - \gamma$ can then be used to inform a higher-level mode-sequencing algorithm to defer or discard a proposed mode sequence.

Hsu et al. prove a similar claim to ours for a different problem parametrization referred to as `expansiveness': a lower bound on the fraction of the configuration space that can be connected to an adversarial point with a straight line.
Their results explain the strong performance of the PRM in problems of higher dimension (up to six or seven).
Using the expansiveness parametrization and their bounds for problem feasibility is challenging: in attempting to estimate the expansiveness, one may also be able to solve the motion planning problem as well \cite{hsu_path_1997}.
It is likely that narrow passage width is also formally hard to estimate, but reasonable path widths (as interpreted as `tubes' around feasible paths) can defined given tolerances of the robot's control infrastructure and uncertainty of the environment model used for planning.

%
There are many probabilistic convergence rate results for sampling-based motion planning algorithms, and specifically, for PRMs.
All study probability of finding an existing solution \cite{kavraki_analysis_1998} or near-optimal solutions \cite{dobson_geometric_2015} as a function of the number of samples (e.g. the `sample complexity' of a motion planning algorithm).


==> sections/legacy/from_notes.tex <==
% From research notes: June1st-5th when we were first proving the result that we wish Tsao gave us
\begin{definition}
    Let $\mathcal X \subset \R^n$. A finite subset $N \subset \mathcal X$ is a geometric $\epsilon$-net of $X$ if for every $x \in \mathcal X$ there exists $x_n \in N$ such that $||x - x_n||_2 \leq \epsilon$.
\end{definition}

\begin{remark}
    Technically, $\epsilon$-nets are defined with respect to a norm. Here, we take the Euclidean norm (but sometimes, it's more convenient to take the $\infty$-norm, for example.
\end{remark}

We take the combinatorial definition from \cite{matousek_lectures_2002}.
\begin{definition}
    Let $\mathcal X$ be a (potentially infinite) compact set, and let $\mu$ be a measure on $\mathcal X$. Suppose $(\mathcal X, \mathcal F)$ be a set system such that every $S \in \mathcal F$ is measureable with respect to $\mu$. A finite subset $N \subset \mathcal X$ is a combinatorial $\epsilon$-net if for all $S \in \mathcal F$ such that $\mu(S) \geq \epsilon \cdot \mu(\mathcal X)$, then $N \cap S \neq \emptyset$.
\end{definition}

The geometric $\epsilon$-net is more convenient for finding relative-optimality bounds for path solutions for PRMs, while the combinatorial $\epsilon$-net is the construction that theoretical learning-theorists/computational geometers/combinatorialists use for algorithmic constructions. Here's the connection between the two objects:

For now, (for simplicity) let's assume (given an appropriate scaling) that $\mathcal X$ is always scaled so that its volume is 1.

\begin{lemma}\label{lem:geom_e-net_iff_comb_e-net}
    Let $\mathcal X \subseteq \R^d$, and $\mu$ be the Lebesgue measure (and assume $\mu(\mathcal X) = 1$). Let $N \subset \mathcal X$ be a finite subset. $N$ is a geometric $\epsilon$-net of $\mathcal X$ if and only if $N$ a combinatorial $\epsilon^d\mu(B_2^d(1))$-net on the set system $(\mathcal X, \mathcal F)$ where $\mathcal F$ is the set of all $l_2$-balls in $\mathbb R^d$ that have non-empty intersection with $\mathcal X$.
\end{lemma}

\begin{proof}
   This proof does not contain a lot of insight, just going from one definition to the other.

   We start with the forward direction. Suppose $N$ is a geometric $\epsilon$-net. Let $S \in \mathcal F$ such that $|S| \geq \epsilon^d \mu(B_2^d(1))$ (i.e., $S$'s volume is larger than that of a $d$-dimensional ball with radius $\epsilon$). Since $S$ is a ball, its radius must be larger than $\epsilon$. Let $x_S$ be its center. By the definition of geometric $\epsilon$-net, there exists $x_n \in N$ such that $||x_c - x_n|| \leq \epsilon$, so $x_n \in S$.

   The backward direction is even quicker. Let $N$ be a combinatorial $\epsilon^d B_2^d(1)$. Let $x \in \mathcal X$. Let $S$ be the $d$-dimensional ball centered at $x$. Then there must exist $x_n \in N$ such that $x_n \in S$, so $||x - x_n|| \leq \epsilon$.
\end{proof}

\begin{remark}
    The only difference between the `radius' of both nets is accounting for the volume of the $d$-dimensional ball $\mu(B_2^d(1))$. The $\epsilon^d$ constant scales to the ball with radius $\epsilon$.
\end{remark}

Another important fact that we'll use is that the VC-dimension of $([0, 1]^d, \mathcal F)$ is $d + 1$ (according to \cite{mustafa_sampling_2022}).

Theoretical computer scientists/combinatorialists/learning theorists have done lots of work in the 90's and 2000's for constructing (small) $\epsilon$-nets. Learning theory also wants to know the likelihood that small $\epsilon$-nets exist given a uniform sample. Here, we state a result by \cite{blumer_learnability_1989} that hands us this clincher on a silver platter. There are tighter results out there, but they haven't been phrased with a failure probability. I'm working on trying converting the tightest result out there (\cite{komlos_almost_1992}) into a `failure' probability, but I haven't got those details worked out perfectly yet. Blumer et al. state this theorem in terms of Valiant-style learning theory language (hypothesis spaces, concept classes, etc). We convert it back to combinatorics:

\begin{theorem}\label{thm:blumer_e_net_bound}
   Let $(\mathcal X, \mathcal F)$ be a set system with VC-dimension $d$ and  $\mathcal X \subset \R^n$. Let $\mu$ be a probability distribution on $X$ such that all $S \in \mathcal F$ is measurable with respect to $\mu$. Let $N \subset \mathcal X$ be a set of $m$ independent random samples of $\mathcal X$ with respect to $\mu$, where

   $$
   m \geq \max \curlyb{
    \frac 4 \epsilon \log \frac 2 \delta,
    \frac {8d} \epsilon \log \frac {13} \epsilon
   },
   $$

    then $N$ is a (combinatorial) $\epsilon$-net of $\mathcal X$ with probability at least $1-\delta$.
\end{theorem}



Tsao's contribution (which was a small part of a full theorem proof) the lemma below:

\begin{lemma}\label{lem:tsao_e-net_is_rel_opt}
Let $\mathcal X \subset [0, 1]^d$ be a configuration space, and let $\epsilon > 0$ (to simplify matters, re-scale $\mathcal X$ so that $\mu(\mathcal X) = 1$, where $\mu$ is the Lebesgue measure).
Suppose that $N \subset \mathcal X$ is a (geometric) $\frac{\delta \epsilon}{\sqrt{1 + \epsilon^2}}$-net of $\mathcal X$. Suppose we choose connection radius $r = 2(\alpha + \sqrt{1 - \alpha^2} \delta)$. Then for all $\delta$-clear planning problems $(\mathcal X, x_0, x_g)$, the induced graph on $N$ as constructed by $PRM$ will contain an $\epsilon$-relative optimal path from $x_0$ to $x_g$.
\end{lemma}

We can now put all of our results together to get our first attempt at a sample bound:

\begin{theorem} \label{thm:rough_sample_bound}
 Let $\mathcal X \subset \mathbb R^d$ be a configuration space, and let $\epsilon, \delta, \gamma > 0$ (to simplify matters, re-scale $\mathcal X$ so that $\mu(\mathcal X) = 1$, where $\mu$ is the Lebesgue measure). Suppose that $(\alpha \delta \mu(B^d_2(1)))^d \leq \frac 1 2$.
 Let $\PP$ be the uniform probability measure on $\mathcal X$ (we assume that $\mathcal X$ is a Borel set). Let $N \subset \mathcal X$ be a set of $m$ independent random samples of $\mathcal X$ with respect to $\PP$, where  
 $$
   m \geq \max \curlyb{
    \frac 4 {(\alpha\delta)^d \mu(B_2^d(1))} \log \frac 2 \gamma,
    \frac {8(d + 1)} {(\alpha\delta)^d \mu(B_2^d(1))} \log \frac {13} {(\alpha\delta)^d \mu(B_2^d(1))}
   }.
$$
for $\alpha = \epsilon / \sqrt{1^2 + \epsilon^2}$. Then for all $\delta$-clear planning problems $(\mathcal X, x_0, x_g)$, the induced graph on $N$ as constructed by $PRM$ will contain an $\epsilon$-relative optimal path from $x_0$ to $x_g$ with probability at least $1 - \gamma$.
\end{theorem}

\begin{proof}
    We know from \cite{mustafa_sampling_2022} that the VC-dimension of $(\mathcal X, \mathcal F)$ is $d + 1$.
    By Theorem \ref{thm:blumer_e_net_bound}, we know that $N$ is a combinatorial $(\alpha\delta)^d\mu(B_2^n(1))$-net of the set system $(\mathcal X, \mathcal F)$ (where $\mathcal F$ is the set of Euclidean balls in $\R^d$) with probability at least $1 - \delta$.
    By Lemma \ref{lem:geom_e-net_iff_comb_e-net}, we know that $N$ is a geometric $\alpha\delta$-net with probability at least $1 - \delta$. 
    By Lemma \ref{lem:tsao_e-net_is_rel_opt}, we know that the induced graph computed by the PRM algorithm will contain an $\epsilon$-relative optimal path from $x_0$ to $x_g$.
\end{proof}

\subsection*{Comparing to Tsao's Result}
It's hard to compare the rates directly, but in his results, Tsao uses a union-bound-volume based upper bound on $\epsilon$-nets to find nets of $O\paren{(\frac{\epsilon + 1}{C})^d \frac{d^{\frac{d+1}{2}}}{\epsilon^d}}$. For $C > 1$. Our bound translates Welzl + Haussler's probabilistic construction $O\paren{\epsilon^{-d}d^{\frac{1-d}{2}} \log \epsilon^{-d} d^{\frac{-(d+1)}{2}}}$. We need to compare these! I would hope ours is tighter.

% from trying to formalize TAMP as a motion-planning problem. (6/27 onwards)

\section*{Posing a Simple TAMP Problem}

Our objective here is to understand the orbit-selection component of Will's problem. Our toy problem is going to need to capture two fundamental features:

\begin{enumerate}
    \item We we choose an orbit, we `commit' to it and will have to move to a boundary to switch.
    \item Long term consequences of actions/orbit selection.
\end{enumerate}

The manifold structure of each orbit/mode seems to be an orthogonal feature, and we'll study its complications after we develop some more maturity in the subject. We'll model our current problem as a bunch of copies of $\mathbb R^n$ of varying dimension glued together at the boundary.

The toy problem I have in mind looks something like:

The problem statement is modified directly from \cite{goldberg_asymptotically_2020}. We're purposefully omitting velocities from the state, since the dynamics may complicate the problem we are trying to solve here.

Let $\mathcal X$ be a fully-connected configuration space with flat metric structure. Suppose that $\mathcal X$ is the zero-level set of $f: \R^d \times T(\R^d) \to \R$, in some embedding space $\R^d$. A continuous feasible path $\sigma: [0, 1] \to \mathcal X$ can then be represented by $\sigma: [0, 1] \to \R^d$ and $g(\sigma(t)) = 0, \forall t \in [0, T]$. Suppose $(x_0, \mathcal X_g)$, be a tuple of a initial state and goal state of the planning problem. The cost of the planning problem is the length of the feasible path $\sigma$.

Suppose $\mathcal X$ has decomposition $\mathcal X = \cup_i \mathcal X_i$ such that $\mathcal X_i \subset \mathbb R^{d_i}$, where $\mathcal X_i$ is manifold with a flat metric and $\mathcal X_i \cap \mathcal X_j$ is either the empty set or a manifold with a flat metric, and that $f$ restricted to $\mathcal X_i$ is analytic. Given $x \in \mathcal X_i$, denote the reachable configurations starting at $x$ as $O_{\mathcal X_i}(x)$, called the orbit. Orbits are pairwise disjoint and are the same dimension. Moving from one orbit to the next on $\mathcal X_i$ will require travelling along its border (which should be/have orbits themselves). \textit{This part will need to be made more rigorous with readings on striations, though Will's paper also goes light on the details too.}

\subsection*{Sampling on Spaces with Mode-Orbit Decompositions}

To understand what a covering argument might look like at the manifold boundary (the thing I'm worried about is the behavior of balls that sit cover both orbits where the block is moved far enough for the robot to pass/not moved far enough for the robot not to pass), we need to know two things: (1) the behavior of Will's algorithm at the boundaries of modes and (2) how his proof addresses it (in detail!). 

Two free parameters: $\nu \in (0, 1)$ and $\eta \in (0, \infty)$.
\subsection*{WVB's Sampling Procedure (paper)}
Some notation: $O_{\mathcal X}(x)$ will represent the orbit of $x$ on manifold $\mathcal X$.
    \begin{enumerate}
        \item Construct a priority queue to select lowest-cost vertex.
        \item Remove $x$ from priority queue, then for each mode $\mathcal X_i \ni x$:
        \begin{enumerate}
            \item If $O_{\mathcal X_i}(x)$ does not contain any samples:  Sample $n$ times from $O_{\mathcal X_i}(x)$
            \item For each mode $\mathcal X_i'$ s.t. $\mathcal X_i' \cap \mathcal X_i \neq \emptyset$, sample the boundary $\nu n$ times to generate $\nu n$ samples at $O_{\mathcal X_i}(x) \cap \mathcal X_i'$.
        \end{enumerate}
    \end{enumerate}

Distances to connect points are measured using distance defined by the current mode containing the current orbit (and must agree on boundary points). They are lazily evaluated using A*.

\begin{definition}
        A path $\sigma$ is $\delta$-decision clear if for all $0 \leq t \leq 1$ and for all $i$ such that $O_{X_i}(\sigma(t))$ is non-empty:
        
        $O_{X_i} - \{B^2_\delta(\sigma(t)): \forall t \in [0, 1] \}$ does not contain a path homotopic to $\sigma$ in quotient space $X \backslash X_g$ (e.g. space we get by gluing the goal set together) containing $y$.
\end{definition}

\begin{remark}
   We may need to put some technical conditions on the goal set $X_g$ for well-behaveness. We need to explore if we fix a single state space if this definition returns back to the single state space. 

   This definition allows us capture the whole homotopy class of solution, with some geometric grounding.

   The quotient part of the definition is there to make sure we have a well-defined idea of homotopy when reaching the abstract `goal' (so we just crunch the goal set down into a point).
\end{remark}

With this definition, we can probably do within-homotopy-class `completeness-type' bound pretty easily, should we be able to bound the number of mode transitions to a finite set:

\begin{theorem}
    Let $\mathcal X \subset \mathbb R^d$ be a configuration space and $f: \mathcal X \times T \mathcal X \to \R$ be a constraint function that induces a stratified decomposition of $\mathcal X$ as in the problem definition above. Let $x_0 \in \mathcal X$ be an initial state and $X_g \subset \subset \mathcal X$ be a set of goal states.
    
    Let $\sigma^* [0, 1] \to \mathcal X$ be an admissable $\delta_o$-obstacle clear and $\delta_d$-decision clear optimal path. Suppose that $\sigma^*$ passes through a FINITE number of orbits, i.e. $k$ orbits. 

    Suppose that $S$ is a set of samples derived from a $(N, M, k)$-run of Will's sampling scheme above. If $S$ forms a $\delta_d$-net on all orbits contained in boundaries of modes, and $S$ forms a $\delta_o$-net on all orbits that are not contained in bound, then the induced graph on $S$ with an unbounded connection radius will contain a path from $x_0$ to $X_g$ in the same homotopy class as $\sigma^*$.
\end{theorem}









==> sections/legacy/numerical_bound_alg.tex <==
While Theorem \ref{thm:rough_sample_bound} states an argument for how the sample complexity should scale with respect to clearance, optimality tolerance, and failure, the actual sample quantity the bound calls for is loose. 
In practice, to obtain a better estimate of the sample complexity, we perform a numerical search on the earliest computable quantity in Blumer et al.'s  proof \cite{blumer_learnability_1989}. 
We reproduce an abridged version of the argument \footnote{A fantastic exposition of Vapnik and Chervonenkis' argument can be found in Matousek's \textit{Lectures on Discrete Geometry}   \cite{matousek_lectures_2002}.}, adapted to our application of hitting $d$-dimensional balls of volume at least $\rho$ in the robot's configuration space $X$ with a set of i.i.d samples $N$:
\begin{align}
    &\mathbf P(N \text{ is not a } \rho\text{-transversal.})\\
    =&\mathbf P(\exists B_2^d \mbox{ s.t. } \mu(B_2^d) \geq \rho \mbox{ and } N \cap B_2^d = \emptyset) 
    &&\text{(Defn. $\epsilon$-transversal)}\\
    \leq& \underbrace{
        \paren{
            \sum_{i=1}^{d+1} \binom{2|N|}{i}}
        }_{O(m^{d+1})} \cdot 2^{-\epsilon |N|/2}
    &&\text{(Sauer-Shelah lemma, etc.)} \\
    \leq& \textit{ ...additional bounds for a closed form rate...}
\end{align}

We compute $\rho = \PP(B^d(\frac{\epsilon \delta}{\sqrt{1 + \epsilon^2}}))$ as done in Theorem \ref{thm:rough_sample_bound}, and evaluate the third line of the (regrettably) abridged argument as \textsc{ComputeVCBound($N$)}.\footnote{For brevity, we only including the number of samples $N$ as an argument, since the other parameters in the expression are fixed in a single motion planning problem instance.}
Because the first term in the third line is strictly increasing in $|N|$ and the second is strictly decreasing in terms of $|N|$, we can find a tight estimate of the samples required using a simple numerical search.
We use doubling-scheme to find a bounding interval of the tightest sample count past `hump' of the probability bound and binary search on the interval afterwards (Algorithm \ref{alg:numerical_complexity}).
We find that numerically searching over a tigher term in Blumer's proof yields a significantly tighter estimate relative of the given bound (Figure \ref{fig:theory-vs-numerical-transversal}).

\begin{algorithm}[h]                \caption{\textsc{NumericalBound}}\label{alg:numerical_complexity}
    \begin{algorithmic}[1]
        \Require $1 > \gamma > 0$
        \State $N_l \gets 1$, $N_u \gets 1$
        \While{$\textsc{ComputeVCBound}(N_u + 1) < \textsc{ComputeVCBound}(N_u) < \gamma$}
            \State $N_u \gets 2N_u$ 
            \Comment{Find interval that contains desired sample count.}
        \EndWhile
        \While{$N_l + 1 < N_u$}
            \State $N_{mid} \gets \floor{(N_l + N_u) / 2}$
            \If{$\textsc{ComputeVCBound}(N_{mid} + 1) < \textsc{ComputeVCBound}(N_{mid}) < \gamma$}
                \State $N_u \gets N_{mid}$  \Comment{Binary search to find the tightest sample count.}
            \Else
                \State $N_l \gets N_{mid}$
            \EndIf
        \EndWhile\\
        \Return{$N_u$}
    \end{algorithmic}
\end{algorithm}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{example-image}
    \caption{A comparison of the sufficient number of samples required to find an $\epsilon$-transversal as shown by Theorem \ref{thm:blumer_e_net_bound} and numerical computation done by Algorithm \ref{alg:numerical_complexity}.}
    \label{fig:theory-vs-numerical-transversal}
\end{figure}




==> sections/legacy/orbt.tex <==
We use Vega-Brown and Roy's \cite{goldberg_asymptotically_2020} construction of the MMMP problem and will  analyze the sampling strategy of their Orbital-Bellman Tree (OBT) algorithm\footnote{\sas{We'll get to Factored-OBT once we have intuition about OBT here!}}, an asymptotically optimal modification of PRM* for multi-modal problems.

\subsection{MMMP Problem Construction}
In multi-modal motion planning problems, the discrete planning structure is introduced by natural constraints that model \textit{contact}. 
A simple example is the following:

\begin{equation}\label{eqn:example_mmmp_constraint}
f_{\text{contact}}(x_{\text{robot}}, x_{\text{object}}, v_{\text{robot}}, v_{\text{object}}) 
= v_{\text{object}}^2 \cdot \mathbb I_{\text{in-contact}}(x_{\text{robot}}, x_{\text{object}}) 
\end{equation}

\noindent which should be read as "the object does not move, or the object and robot are in contact."

We express the configuration and velocity space (e.g. the tangent bundle of the configuration space) of a robot and its manipulable objects $\mathcal X \times T(\mathcal X)$ as the zero-level set of a constraint function $f: \R^n \times T(\R^n) \to \R$, such as the one above (the [curly font] is used to indicate that $\mathcal X$ may have non-Euclidean).  
A feasible path $\sigma: [0, 1] \to \mathcal X \times T(\mathcal X)$ must also obey the constraint function as well ($f(\sigma(t)) = 0$ for $0 \leq t \leq 1$).

$\mathcal X$ can be decomposed into modes, which are subsets $\mathcal X_i \subset \mathcal X$ where $f$ restricted to $\mathcal X_i$ and $T(\mathcal X_i)$ is \textit{analytic}. 
We know from differential geometry \cite{tu_introduction_2011}  that all $\mathcal X_i$ admit manifold structure,  and the union of all modes is the full configuration space $\mathcal X$. 
We assume that there are a finite number modes and that they are all \textit{flat} manifolds (do not have intrinsic curvature).\footnote{\sas{I am making this assumption because sampling uniformally on curved spaces is strange\cite{diaconis_sampling_2013}. Since the curvature is really a detail here, I'm treating the flat case first, and will generalize later once I have a set of results.} }

Modes themselves can be decomposed into \textit{orbits}, which are the reachable configurations from a chosen point $x \in \mathcal X_i$. 
The Froebenius theorem \cite{tu_introduction_2011} tells us that orbits form a partition of a mode $\mathcal X_i$, also admits manifold structure, and all have the same dimension.\footnote{In differential topology, a mode is also known as a \textit{striation} and the orbits known as \textit{leaves} or \textit{strata}.}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{assets/pusher_example_problem.png}
    \caption{An example domain where the robot must grasp and push the block out of the way to clear the shortest path to the goal, with constraints in the form of Equation. \ref{eqn:example_mmmp_constraint}.}
    \label{fig:block_mmmp_example}
\end{figure}

An example of the definitions above can be found in the block-pushing domain described in Figure \ref{fig:block_mmmp_example}, with constraints taking the form of the example Equation \ref{eqn:example_mmmp_constraint}. 
There are two modes: the mode where the robot is \textit{in contact} with the block, and the mode where the robot is freely moving around without the block.
On the contact mode, the orbits are indexed by the robot's grasp pose, and on the free-movement mode, the orbits are indexed by the pose of the block.

A multi-modal motion planning problem is defined by a configuration space $\mathcal X$ and a mode-orbit decomposition induced by a constraint function $f:\R^n \times T(\R^n) \to \R$.
We wish to compute a path from a specified initial state $x_0 \in \mathcal X$ to a set of goals $X_g \subset \mathcal X$, minimizing the distance travelled by the robot.\footnote{Vega-Brown and Roy consider the more general MMMP problem where $c$ may not just be distance traveled by the robot.} 

\subsection{Orbital-Bellman Sampling Procedure}\label{sec:orb-t_sampling}

The robot can only travel to points that share the same orbit, and so we must grow our roadmap orbit-by-orbit instead of randomly sampling from the whole of $\mathcal X$.
To ensure path-connectivity, OBT start its search on one orbit and ensures that neighboring orbits are visited.
The sampling procedure has two free parameters: $\nu \in (0, 1)$ and $\eta \in (0, \infty)$. 
We denote the orbit containing $x \in \mathcal X$ on mode $\mathcal X_i$ as $O_{\mathcal X_i}(x)$. 
We briefly sketch the sampling procedure below, which continues until the a point in the goal set $X_g$ is found:

\begin{enumerate}
    \item Construct a priority queue to select lowest-cost vertex, where priority is defined by the current length of the path to each vertex.
    \item Remove $x$ from priority queue, then for each mode $\mathcal X_i \ni x$:
    \begin{enumerate}
        \item If $O_{\mathcal X_i}(x)$ does not contain any samples:  Sample $n$ times from $O_{\mathcal X_i}(x)$. 
        \item For each mode $\mathcal X_i'$ s.t. $\mathcal X_i' \cap \mathcal X_i \neq \emptyset$, sample the boundary $\nu n$ times to generate $\nu n$ samples at $O_{\mathcal X_i}(x) \cap \mathcal X_i'$.
    \end{enumerate}
    We refer $x$ as the \textit{parent} of any of the points sampled at this step.
\end{enumerate}

In addition to the number of samples for orbit $n$, we also need to identify the number of times the search process explores a new orbit.
If $x$ is the parent of the parent of sampled point $x'$, then we say $x$ is the 2-parent of $x$. 
$k$-parents for positive integer $k$ is defined in a similar fashion.
We say that the the sampling procedure has \textit{proceeded through $k$ orbit levels} if for every point in the priority queue $x$, the starting configuration $x_0$ is at least the $k$-parent of $x$.


\subsection{Defining Optimality for MMMP Problems}

Since every orbit in an MMMP problem is a space that is treated as a traditional motion planning problem, we will still use all of the terminology we introduced in Section \ref{sec:complexity_mp}.
However, the discrete mode-switching component of MMMP forces us to consider a new type of clearance, unrelated to the obstacles.
Intuitively, this clearance refers to the ease of a sampling-procedure to find orbits that are close to the one chosen by the optimal algorithm.

\begin{definition}
        Let $\sigma:[0, 1] \to \mathcal X$ be a feasible path. 
        Suppose there there exists a set $D$ of positive reals such that for all $\delta \in D$, $0 \leq t \leq 1$, and $i$ such that $O_{X_i}(\sigma(t))$ is non-empty:
        
        $O_{X_i} - \{B^2_\delta(\sigma(t)): t \in [0, 1], \sigma(t) \in \partial O_{X_i}(\sigma(t)) \}$ does not contain a path homotopic to $\sigma$ in quotient space $X \backslash \paren{\{X_g\} \cup \{\{x\} \in \mathcal X: x \notin X_g \}}$  containing $y$.\footnote{The quotient is a technical operation to ensure that the paths we are homotoping have a well-defined end-point, but does bear any weight for any of the upcoming discussion.} If $\delta = \inf D > 0$, then we say that $\sigma$ is $\delta$-decision clear.
\end{definition}

A way to intuit this definition is to think that $\delta$ quantifies the size of the space that must be removed from the orbit so that the sampling algorithm would not be able to discover paths that are close to optimal (e.g. "make the right decisions").
A depiction of the decision-clearance for the block-pushing example shown above can be found in Figure \ref{fig:decision-clearance-ex-mmmp}.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{assets/decision_clearance.png}
    \caption{Decision clearances on orbits on the grasping mode.}
    \label{fig:decision-clearance-ex-mmmp}
\end{figure}

The orbit-mode decomposition of $\mathcal X$ prevents us from defining a computationally tractable global optimality condition analogous to $(\epsilon, \delta)$-completeness, since there is potentially an uncountable number of orbits in each mode.
Instead, we can only focus on a single MMMP problem from a single $x_0$ to $X_g$. 

\begin{definition}
    Let $\mathcal X$ be a configuration space, and let $N \subset \mathcal X$ be the set of samples produced by the sampling scheme outlined in \ref{sec:orb-t_sampling}. $(\mathcal X, x_0, X_g, N, r)$ is $(\delta, \epsilon)$-decision complete if
    $$
    \text{shortest path length in graph built by OBT} < (1 + \epsilon) \cdot c(\sigma^*)
    $$
    where $\sigma^*$ is the optimal $\delta$-decision clear solution path to $(\mathcal X, x_0, X_g)$.
\end{definition}


\subsection{Bounding the Sample Complexity of OBT}
Our proof follows the sample general pattern as presented in Section \ref{sec:complexity_mp}. 
Here, we immediately obtain a result about finding paths that are in the same $\textit{homotopy class}$ as the optimal $\delta$-decision clear path.

\begin{proposition}\label{prop:mmmp_completeness}
    Let $\mathcal X \subset \mathbb R^d$ be a configuration space and $f: \mathcal \R^d \times T (\R^d) \to \R$ be a constraint function that induces a mode-orbit decomposition of $\mathcal X$. Let $x_0 \in \mathcal X$ be an initial state and $X_g \subset \mathcal X$ be a set of goal states.
    
    Let $\sigma^* [0, 1] \to \mathcal X$ be a $\delta_d$-decision clear  and $\delta_o$-(obstacle) clear optimal path. Suppose that $\sigma^*$ passes through a finite number of orbits, i.e. $k$ orbits. 

    Suppose that $S$ is a set of samples derived from a sampling scheme that sampled $N$ points per orbit and progressed through $k$ orbits. 
    If $S$ forms a $\delta$-net on all orbits contained in boundaries of modes with connection radius $r \geq 2\max\{\delta_d, \delta_o\}$, then  graph produced by OBT will contain a path from $x_0$ to $X_g$ in the same homotopy class as $\sigma^*$.
\end{proposition}

\sas{This section is under active development, since not everything has been proved yet! I'm don't have a clear picture of what will be involved in the bound, so this section is going to be left unfinished for now.}


==> sections/legacy/terminology.tex <==
% introduce the machinery, and give an intuition for what it means

Our arguments are centered around covering and point configurations and the probability they arise from random sampling processes, a topic well-studied at the intersection of statistics, combinatorics, and discrete geometry \cite{mustafa_sampling_2022,matousek_lectures_2002}\footnote{We will be using terminology from both computational geometry and statistics to avoid conflicting terminology in the same paper.}. 

Our intuition behind the definitions is grounded in trying to `hit' a class of subsets of some space $X$ with a random finite set of points.

\begin{definition}
   $X$ be a (potentially infinite) set, and let $\F \subset 2^X$. We call the tuple  $(X, \F)$ a range space.\footnote{For those who are familiar with learning theory: another name for $\F$ can be the \textit{hypothesis space} of a set of binary classifiers or set of indicators associated with all elements of $\F$.}
\end{definition}


We will take $X \subset \R^n$ to represent the obstacle-free configuration space of a robot (and possibly a manipulable object in the environment).
$\F$ will be the set of $n$-dimensional balls that are a proper subset of $X$. 

Often, hitting $\textit{all}$ the sets in $\F$ with a finite number of points in $X$ is too tall an order to ask. 
For our purposes, only hitting the `voluminous' sets in $\F$ is enough.

\begin{definition} \label{def:e-transversal}
    Let $(X, \F)$ is a range space. Suppose that $\mu$ is a measure on $\mathcal X$ such that every $S \in \mathcal F$ is measureable with respect to $\mu$. 
    
    A finite subset $N \subset X$ is an $\epsilon$-transversal if for all $S \in \mathcal F$ such that $\mu(S) \geq \epsilon \cdot \mu(X)$, then $N \cap S \neq \emptyset$.
\end{definition}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{assets/epsilon_transversal.png}
    \caption{An example of an $\epsilon$-transversal of disks on a plane, where $\epsilon$ is set larger than the volume of the two small disks at the bottom.}
    \label{fig:e-transversal}
\end{figure}

Intuitively, $\epsilon$ is a \textit{threshold} on the minimum volume of  $S \in \F$ to be hit by a point in $N$. 
There could be many different $\epsilon$-transversals on $(X, \F)$, and we prefer to find smaller $\epsilon$-transversals if we can. 
An example  is depicted in Figure \ref{fig:e-transversal}. But how do we construct an $\epsilon$-transversal? 

Blumer et al. \cite{blumer_learnability_1989}, generalizing Welzl and Haussler's  work \cite{haussler_epsilon-nets_1986}  from discrete to continuous range spaces\footnote{The original proof technique is credited to Vapnik and Chervonenkis \cite{vapnik_uniform_1971}.} showed that random sampling can find $\epsilon$-transversals with high probability.

\begin{theorem}\label{thm:blumer_e_net_bound}
   Let $(\mathcal X, \mathcal F)$ be a range space with VC-dimension $\VC(\F)$ and  $\mathcal X \subset \R^n$. 
   Let $\PP$ be a probability distribution on $X$ such that all $S \in \mathcal F$ is measurable with respect to $\PP$. 
   
   Let $N \subset \mathcal X$ be a set of $m$ independent random samples of $\mathcal X$ with respect to $\PP$, where
   $$
   m \geq \max \curlyb{
    \frac 4 \epsilon \log \frac 2 \gamma,
    \frac {8d} \epsilon \log \frac {13} \epsilon
   },
   $$
    
    \noindent then $N$ is an $\epsilon$-transversal of $\mathcal X$ with probability at least $1-\gamma$.
\end{theorem}

\noindent 
Intuitively, the VC-dimension is a quantification of the \textit{complexity}, or intricacy, of the ways the sets in $\F$ intersect with $X$ and each other (see Appendix).
Our arguments only require the fact that the VC-dimension of a set of $d$-dimensional (Euclidean) balls in $\R^d$ is $d+1$ \cite{matousek_lectures_2002,mustafa_sampling_2022}. 
The right argument of the maximization makes a statement on the size of \textit{small} $\epsilon$-transversals, e.g. we can find small $\epsilon$-transversals near-linearly in $1/\epsilon$ and linearly in $d$.
The left allows us to make an estimate on the probability of failure $\gamma$. 

While this theorem provides us with an understanding of how samples should scale with the parameters of an $\epsilon$-transversal, in practice, the looseness introduced by the maximum operation does not immediately translate to practical computations of sample $m$. 
Later, we will introduce a numerical algorithm based on the proof of Theorem \ref{thm:blumer_e_net_bound} that will compute a tighter quantity of samples that are sufficient to find an $\epsilon$-transversal given a probability of success.


We name one other type of point configuration, used by Tsao et al. \cite{tsao_sample_2019} , which formalizes the notion of a "covering" set of points.

\begin{definition}\label{def:e-net}
    Let $X \subset \R^n$. A finite subset $N \subset X$ is an $\epsilon$-net of $X$ if for every $x \in X$ there exists $x_n \in N$ such that $||x - x_n||_2 \leq \epsilon$.
\end{definition}

\noindent
This definition can be interpreted as a covering of a space $X$ with balls with radius $\epsilon$, whose centers are the points in the $\epsilon$-net.

When uniformly sampling from a space $X \subset \R^n$, we are in a favorable scenario where $\epsilon$-transversal (hitting set of balls in $X$)  $\epsilon$-net (covering $X$ with balls)  coincide.

\begin{lemma}\label{lem:geom_e-net_iff_comb_e-net}
    Let $X \subseteq \R^d$, and $\PP$ be a uniform probability measure. 
    Let $N \subset \mathcal X$ be a finite subset. 
    
    $N$ is an $\epsilon$-net of $X$ if and only if $N$ is an  $\epsilon^d\PP(B^d(1))$-transversal on the range space $(X, \mathcal F)$ where $\mathcal F$ is the set of $d$-dimensional balls in $\mathbb R^d$ that have non-empty intersection with $X$.
    We denote a $d$-dimensional ball with radius $r$ as $B_2^d(r)$\footnote{The 2 refers to the $\ell_2$ norm.}.
\end{lemma}
\begin{proof}
   % This proof is not very insightful; we are taking advantage of the fact that the volume of a sphere coincides with the probability we sample from it under the uniform probability measure.

    %   Let $\mu$ be the Lebesgue measure. Let $\lambda = \PP(B^d(1)) / \mu(B^d(1))$, i.e. the scale factor between the uniform and Lebesgue measure.
    % We actually don't need to relate these two quantities, especially if they are just off by a contsant factor
    The essence of this proof is a radius-volume conversion, which is only possible since we are working with range spaces with spheres.
   
   We start with the forward direction. 
   Suppose $N$ is an $\epsilon$-net. 
   Let $S \in \mathcal F$ such that $\PP(S) \geq \epsilon^d \PP(B_2^d(1)) \cdot \PP(X) = \epsilon^d \PP(B_2^d(1))$ (i.e., $S$'s volume is larger than that of a $d$-dimensional ball with radius $\epsilon$). 
   Since $S$ is a ball, its radius must be larger than $\epsilon$. Let $x_S$ be its center. 
   By the definition of geometric $\epsilon$-net, there exists $x_n \in N$ such that $||x_c - x_n|| \leq \epsilon$, so $x_n \in S$.

   The backward direction is even shorter. Let $N$ be a $\epsilon^d \PP(B_2^d(1))$-transversal. 
   Let $x \in \mathcal X$. Let $S$ be the $d$-dimensional ball centered at $x$. 
   Then there must exist $x_n \in N$ such that $x_n \in S$, so $||x - x_n|| \leq \epsilon$.
\end{proof}



